Reproducible, incremental representation learning with Rosetta VAE

Variational autoencoders are among the most popular methods for distilling low-dimensional structure from high-dimensional data, making them increasingly valuable as tools for data exploration and scientific discovery. However, unlike typical machine learning problems in which a single model is trained once on a single large dataset, scientific workflows privilege learned features that are reproducible, portable across labs, and capable of incrementally adding new data. Ideally, methods used by different research groups should produce comparable results, even without sharing fully trained models or entire data sets. Here, we address this challenge by introducing the Rosetta VAE (R-VAE), a method of distilling previously learned representations and retraining new models to reproduce and build on prior results. The R-VAE uses post hoc clustering over the latent space of a fully-trained model to identify a small number of Rosetta Points (input, latent pairs) to serve as anchors for training future models. An adjustable hyperparameter, $\rho$, balances fidelity to the previously learned latent space against accommodation of new data. We demonstrate that the R-VAE reconstructs data as well as the VAE and $\beta$-VAE, outperforms both methods in recovery of a target latent space in a sequential training setting, and dramatically increases consistency of the learned representation across training runs.

==> sections/experiments_simplicity.tex <==
To examine the latent embeddings further, we asked how distorted learned maps were across the various models and training runs by asking how close the learned $\mathbf{A}$ matrix in (\ref{eqn:distortion}) is to the identity. Models that best recapitulate the latent space should have $\mathbf{A} \approx \mathbbm{1}$. To investigate this, we performed a polar decomposition, $\mathbf{A} = \mathbf{U} \mathbf{P}$, with $\mathbf{U}$ an orthogonal matrix and $\mathbf{P}$ symmetric positive semi-definite. In Figure \ref{fig:f4}, we plot the eigenvalue spectra for $\mathbf{P}$ for each model type. In all but the 8 Gaussians case, the spectra exhibit an abrupt drop, identifying an effective dimensionality for the data set. Moreover, in each case, the R-VAE exhibits the flattest spectrum, indicating less non-uniform stretching and compression of the learned space relative to the joint training template. We further investigate this by defining $\mathbf{\tilde{A}} = \mathbf{A}/\lVert \mathbf{A}\rVert_\infty$ to be the linear transformation with maximum rescaling of 1. That is, if the two latent spaces are the same up to a global rescaling, we should expect $\mathbf{\tilde{A}} \approx \mathbbm{1}$. In the bottom row of Figure \ref{fig:f4}, we show the quality of this approximation across different models and training runs. Just as in Table \ref{table:t2}, the R-VAE shows lower distortion than both the VAE and $\beta$-VAE with the exception of birdsong, where the results are comparable. Moreover, the biases $\mathbf{b}$ are likewise small (Appendix \ref{app:learned_biases}).

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/f4_final_4x.png}
    \caption{\textbf{Linear transformations between latent spaces are simplest for the R-VAE.} \textbf{First two rows:} Plots of the eigenvalues of the positive semidefinite matrix from polar decomposition of $\mathbf{A}$. In each case, the R-VAE exhibits the flattest spectrum, suggesting only a global rescaling without skew. \textbf{Bottom row:} Norm of the difference between the identity matrix and a version of $\mathbf{A}$ rescaled to have maximum singular value 1. The R-VAE has smaller values, indicating that less linear transformation is needed to align latent spaces found by sequential training.
   }
    \label{fig:f4}
\end{figure}
